Secure Cloud-Edge Deployments, with Trust

Assessing the security level of IoT applications to be deployed to heterogeneous Cloud-Edge infrastructures operated by different providers is a non-trivial task. In this article, we present a methodology that permits to express security requirements for IoT applications, as well as infrastructure security capabilities, in a simple and declarative manner, and to automatically obtain an explainable assessment of the security level of the possible application deployments. The methodology also considers the impact of trust relations among different stakeholders using or managing Cloud-Edge infrastructures. A lifelike example is used to showcase the prototyped implementation of the methodology.

==> notes.tex <==
\subsection{Extending the Embedded Trust Model}



\begin{figure}[ht]
    \Centering
            \begin{Verbatim}[fontsize=\footnotesize]
                trusts(X,X).                    (1)
                                                (2)
                trusts(A,B) :-                  (3)
                    dir(A,B),                   (4)
                    directly_trusts(A,B).       (5)
                trusts(A,B) :-                  (6)
                    \+dir(A,B),                 (7)   
                    indirectly_trusts(A,B).     (8)
                                                (9)
                indirectly_trusts(A,B):-        (10)
                    directly_trusts(A,B).       (11)
                indirectly_trusts(A,B):-        (12)
                    directly_trusts(A,C),       (13)
                    indirectly_trusts(C,B).     (14)
            \end{Verbatim}
    \caption{Trust model of {\sf\footnotesize SecFog}.}
    \label{fig:directvsundirect}
\end{figure}

\noindent
\rev{The model of Fig.} \ref{fig:directvsundirect} \rev{requires users to set the {\tt\small dir(X,Y)} predicate, whenever they want that only existing direct trust relations are considered by} \secfog . Indeed, (transitive) indirect trust is only computed for those trust relations that do not feature a {\tt\small dir(X,Y)} `\textit{flag}' set.


\medskip
\example\ As an example, retaking the trust network of Fig. \ref{trustnetworkexample2}, we assume that {\tt\small ispOp} wants to consider only direct trust relations towards {\tt\small cloudOp} (i.e., 0.7). She will simply declare t
